Time Series Representation Models

Time series analysis remains a major challenge due to its sparse characteristics, high dimensionality, and inconsistent data quality. Recent advancements in transformer-based techniques have enhanced capabilities in forecasting and imputation; however, these methods are still resource-heavy, lack adaptability, and face difficulties in integrating both local and global attributes of time series. To tackle these challenges, we propose a new architectural concept for time series analysis based on introspection. Central to this concept is the self-supervised pretraining of Time Series Representation Models (TSRMs), which once learned can be easily tailored and fine-tuned for specific tasks, such as forecasting and imputation, in an automated and resource-efficient manner. Our architecture is equipped with a flexible and hierarchical representation learning process, which is robust against missing data and outliers. It can capture and learn both local and global features of the structure, semantics, and crucial patterns of a given time series category, such as heart rate data. Our learned time series representation models can be efficiently adapted to a specific task, such as forecasting or imputation, without manual intervention. Furthermore, our architecture's design supports explainability by highlighting the significance of each input value for the task at hand. Our empirical study using four benchmark datasets shows that, compared to investigated state-of-the-art baseline methods, our architecture improves imputation and forecasting errors by up to 90.34% and 71.54%, respectively, while reducing the required trainable parameters by up to 92.43%. The source code is available at https://github.com/RobertLeppich/TSRM.

==> sections/questionaire.tex <==

\newpage
\section*{NeurIPS Paper Checklist}



\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our claims in the introduction and abstract are limited to the tasks of time series forecasting and imputation, our utilized benchmark datasets, and compared SOTA methods. The additional task (classification) is only evaluated in the appendix and thus is not part of the claims in the main paper. 
    
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide a \textit{Limitations} section in our work (see~\ref{sec:limitations}), in which we outline current limitations regarding our approach.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not include theoretical results or proofs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide a link to our public repository, which contains the code for the architecture, experimental scripts, and all required modules to reproduce our results, including data preprocessing. In addition, our appendix includes tables with our best-performing pre-trained models for all experiments for the reader to evaluate. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  We provide a link to our public repository, which contains the code for the architecture, experimental scripts, and all required modules to reproduce our results, including data preprocessing.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide a section about the experimental setup in the main paper~\ref{sec:exp_setup}. In addition we provide a detailed listing of hyperparameter ranges in the Appendix~\ref{appendix:exp_imputation1}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We added multiple random run analysis for the imputation and forecasting experiments in the appendix~\ref{appendix:exp_imputation1}~\ref{appendix:exp_forecasting}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: For our imputation and forecasting experiments we provide the model sizes for our own and those of the compared SOTA models. See~\ref{sec:meth:imputation} and \ref{appendix:exp_forecasting} for details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All authors conform, in every respect, with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work does not yield a societal impact.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: To the best of our knowledge, our work poses no risk.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Citations were incorporated to attribute the creators of all utilized datasets. There are no additional assets involved in our work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No assets result from our work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}



==> sections/related_work.tex <==
\newpage\phantom{blabla}
\newpage\phantom{blabla}
\section{Related Work}

% - Umfang: max 3-4 Seiten
% - Storyline: 
% 1) Schaut mal her es gibt die drei Bereiche: Imputation, Classification und Forecasting (am besten auch in der Reihenfolge da Forecasting am stärksten vertreten ist). 
% 2) In den drei Bereichen gibt es einige Ansätze (kurze Vorstellung mit kaum details) und auch Vertreter die Transformer nutzen (etwas mehr Details). 
% 3) Wir machen das jetzt aber anders (cooler) und haben eine Architektur die alles auf einmal kann in dem ein TS model trainiert wird und die einzelnen Tasks weiter trainiert werden (kannst du einfach beim Approach im Motivation Part dir was klauen). 
% 4) Das gabs auch schon im NLP Bereich -> BERT vorstellen ähnlich wie in der MA aber deutlich gekürzt natürlich. 
In the field of automated time series analysis, there are mainly three different types of tasks that can be considered, namely time series imputation, time series classification, and time series forecasting. Since our developed architecture addresses all three of these tasks, each is briefly explained below, including an overview of current approaches from each area. 
The order in which we present the areas corresponds to their relevance and proximity to our methodology, starting with imputation techniques, which are the most distant in relation to our approach, and ending with forecasting, as the related methods are the most prevalent in our work. While we also present some more traditional machine or deep learning approaches in some areas, we pay special attention to transformer-based methods due to their particular relevance to our architecture.  

\subsection{Imputation}
% Imputation:

% 1. Kurze Übersicht geben was es gibt. Mit BRITS starten wie in der MA. Dann eine andere Variante https://proceedings.mlr.press/v108/fortuin20a.html aber auch hier keine Details, nur ein paar Sätze

% 2. Genau das gleiche hier: https://proceedings.neurips.cc/paper/2018/hash/96b9bff013acedfb1d140579e2fbeb63-Abstract.html

% 3. Und hiermit enden: https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9964035

% Beim Imputation part brauchst du am wenigsten in die Details gehen da die Ansätze recht weit weg sind von meinem. Genau das sollte aber eben rauskommen aus der Storyline. 
Times series imputation refers to the task of replacing missing values with reasonable ones that are estimated based on data observed from the environment with the same underlying conditions. 
% BRITS
A well-known example for the imputation of time series data by means of a bidirectional RNN is the BRTIS architecture that was proposed by Cao et al. in 2018~\cite{cao2018brits}. In their approach, the authors use a bidirectional recurrent dynamical system that is capable of handling multiple correlated missing values in time series without any assumption over the data-generating process. To this end, they combine history-based imputation and feature-based imputation in a bidirectional manner, where the first does not make assumptions about any mutual correlations of the features of a time step and the second aims at improving the imputation accuracy by additionally considering feature correlations. The history-based estimation uses a recurrent component and a regression component for the imputation dependent on previous observations of the same feature, while the feature-based estimation takes into account other correlated features at the same time step and is realized by means of constrained parameter matrix. Both the history-based imputation vector and the feature-based imputation vector are merged to form the final imputation estimation by computing a weighted sum of both vectors, where the weight vector is also learned.

% GP-VAE
Instead of processing (multi-variate) time series as a whole, the imputation approach of Fortuin et al.~\cite{fortuin2020gp} first maps the high dimensional time series with missing values into a latent space without missingness that is fully determined, i.e., a lower dimensional representation whose temporal dynamics can be modeled with a Gaussian Process (GP). To this end, they employ deep variational autoencoders (VAEs) with a novel structured variational approximation to be capable of dealing with the presence of missing data. This latent representation does not only capture correlations between features but the temporal information of the remaining time series is also integrated into the representations by means of the structured variational distribution of the inference network. Hence, similar to the idea of BRITS, both the correlated observed features and the rest of the time series are used for the imputation. 

% GAN
Based on another, fundamentally different idea, Luo et al. treat the imputation of missing values as a task of data generation~\cite{luo2018multivariate}. They adopt an RNN cell, namely, a modified gate recurrent unit called GRUI, in a generative adversarial network (GAN) to both learn the overall distribution of incomplete multivariate time series and model their temporal irregularity. For that purpose, they follow a two-phase approach. First, they integrate the GRUI cell into to the discriminator and generator of the GAN to learn the distribution of the dataset, latent relationships between observations with non-fixed time lags, and temporal information. Second, they optimize the random input ``noise'' of the generator so that the produced time series is as close as possible to the original incomplete series and that the generated data's probability of being real is maximized. For the actual imputation, missing values can than be replaced with the generated fake time series of the GAN, which, due to the second phase, should be most similar to the original incomplete time series.

%MTSIT
In 2022, Yıldız et al. proposed an unsupervised auto-encoder model for the joint reconstruction and imputation of multivariate time series~\cite{yildiz2022multivariate}. They train the auto-encoder architecture, which consists of a transformer encoder and a linear decoder module, by stochastically masking and imputing non-missing values. However, instead of masking each time point independently at random, they use a masking pattern that helps the model learn inter-dependencies between different variables on the one hand as well was between the previous and the following segments within individual variables on the other. 
% In productive use? (im Paper: "At evaluation time")
During inference, the auto-encoder is then capable of imputing both real missing and simulated missing values as in training.

\subsection{Classification}
% Classification:
% 1. Kurze Übersicht über aktuellen heißen shit. 
% -> Geht hier nur darum eine Übersicht zu geben. Also wo kommt der Bereich her, welche ML Methoden gabs und was ist gerade aktuell im Bereich neuronale Netze.
% -> Kannst du aus diesem Survey ziehen: https://link.springer.com/article/10.1007/s10618-019-00619-1?sap-outbound-id=11FC28E054C1A9EB6F54F987D4B526A6EE3495FD&mkt-key=005056A5C6311EE999A3A1E864CDA986

Besides imputation, another task of interest is time series classification (TSC), where TSC models are applied to assign new data to one or several predefined classes after they have been trained on a set of labelled time series data in a supervised manner. 
\todo[inline]{@Robert pls check - ich habe hier jeweils ein Bsp aus dem Survey von dir zitiert, auch wenn ich es nicht immer ganz treffend finde (z.B. lines2015time - die haben auch ensembles aus NNs schon getestet)}
Before the era of deep learning, the research community proposed a multitude of traditional machine learning (ML) methods, ranging from the application of nearest neighbor (NN) classifiers in combination with some distance function like Dynamic Time Warping (DTW)~\cite{lines2015time}, via the development of ensemble methods on one or several feature spaces (e.g., ensembles of decision trees~\cite{deng2013time} or of different types of discriminant classifiers like SVMs, decision trees, and NN classifiers~\cite{bostrom2015binary}), to the classification of time series based on short sub-sequences, the so-called time series shapelets~\cite{ye2009time, hills2014classification}. 
% Hive cote nennnen und Gemeinsamkeit: 
However, despite the variety of possible approaches, they share some common properties: First, all of them rely on some notion of distance between two time series (sub-sequences)~\cite{bock2021machine} and second, the majority of techniques include a data transformation phase, where the original time series are converted into a new feature space~\cite{ismail2019deep}. 
Both of these also apply to Hierarchical Vote Collective of Transformation-based Ensembles (HIVE-COTE), an ensemble of 37 different classifiers trained over multiple time series data transformations. The method was proposed by Lines et al. on 2016 and reached SOTA performance for TSC~\cite{lines2016hive}.

\todo[inline]{@Robert: echo-state networks (ESNs) aus der Survey von dir habe ich weggelassen, dafür RNNs sowie attention- und transformer-basierte Ansätze mit teils eigenen Quellen dazu (egal, ob multivariate oder nicht, teils mehrfach genannt zb für GRU und attention)}
In recent years, researchers have begun to use a multitude of different deep learning (DL) techniques for TSC, many of which operate end-to-end, i.e., without requiring a dedicated, manual feature engineering step or domain-specific pre-processing steps~\cite{ismail2019deep}. Successfully applied DL methods for TSC cover multi-layer perceptrons (MLPs)~\cite{wang2017time}, recurrent neural networks (RNNs) such as long short term memories (LSTMs)~\cite{tang2016sequence} or gated recurrent units (GRUs)~\cite{tan2020data}, and convolutional neural networks (CNNs) including fully-convolutional networks (FCNs) and residual networks (ResNets)~\cite{wang2017time}. 
Furthermore, different combinations of CNNs and RNNs such as LSTM-FCN~\cite{karim2019multivariate}, temporal convolutional neural networks (TCNs)~\cite{tang2021channel} and especially, recent developments such as attention-based neural networks (e.g., in~\cite{tang2016sequence, tan2020data, karim2019multivariate, tang2021channel}) or transformer-based architectures~\cite{liu2021gated}\todo[]{arXiv pre-print} are increasingly used for TSC as well. Among current SOTA methods, TapNet~\cite{zhang2020tapnet} and ShapeNet~\cite{li2021shapenet} are two representatives, where the former uses a CNN and LSTM combined with so-called class prototypes for TSC, and the latter is based on a novel shapelet-based neural network. 
\todo[inline]{@Robert: Bin bei der Recherche bzw im Paper von MCTNet auf ShapeNet (shapelet neural network) und TapNet  (attentional prototypical network + Vorlage für MCTNet) als aktueller SOTA gestoßen, habs auch mal noch mit rein}

% 2. An Aggregated Convolutional Transformer Based on Slices and Channels for Multivariate Time Series Classification
%  -> Das Paper hier kannst du dann etwas genauer beleuchten. Allerdings nicht so umfassend. Geht hier nur darum zu zeigen wie Transformer Architekturen in Kombination mit CNNs genutzt werden können für Classification. Also bitte nicht in die Details gehen, das wäre zu aufwändig. https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9918094
However, it is not only possible to combine classical methods such as RNNs or CNNs with each other, as in TapNet~\cite{zhang2020tapnet}, but also to merge them with transformer components to form a hybrid time series classifier. To give an example, Wu et al. proposed a multivariate time series classification convolutional transformer network (MCTNet), where they fused an transformer encoder and convolutional structures into an overall architecture to combine the advantages of both methods~\cite{wu2022aggregated}. 
\todo[inline]{@Robert - ich hatte es erst sehr nahe am Paper (III.A), aber da versteht man finde ich vieles nicht direkt. Hat mich bissl Zeit gekostet bis ichs grob verstanden hatte und habs jetzt teils selbst geschrieben. Pls check)}
To this end, they propose a both squeeze and excitation convolution encoder structure with two branches, namely a channel attention branch and a slice attention branch. The two attention-based feature representations are then fused to a lower-dimensional representation and an attentional class prototype calculation is performed. % passed to a subsequent component for attentional prototype learning
% Nahe am Paper: During test time, a similarity transformer is performed with the obtained class prototype, where the classification result is calculated using a softmax function.
During test time, f(or a new sample, the probability of each class and hence, the class distribution, can be calculated based on the similarity between the low-dimensional representation of the sample and that of each class prototype using a softmax function.

\subsection{Forecasting}
Time series forecasting (TSF) refers to the task of fitting a model to historical and current data in order to estimate future values over a period of time or to predict a certain point in the future. While early approaches for TSF such as Autoregressive Integrated Moving Average (ARIMA) models~\cite{box2015time} or structural time-series models~\cite{harvey1990forecasting} focused on parametric models based on domain expertise, modern deep learning (DL) methods allow to learn temporal dynamics in a purely data-driven manner, i.e., without the need for manual feature engineering~\cite{lim2021time}. Examples of DL architectures for TSF include deep feed forward neural networks, (bidirectional) recurrent neural networks, convolutional neural networks, and attention-based neural networks, with Torres et al.~\cite{torres2021deep} as well as Lim and Zohren~\cite{lim2021time} providing detailed overviews of time-series forecasting with DL.

% MA Robert
\todo[inline]{@Robert - im Folgenden hab ich einen Teil aus deiner MA geklaut (Chapter 3.1). Wo hast du die erste Aussage her? Das Paper, das du in der MA verlinkst, macht dazu eigt keine Aussage auf den ersten Blick: \textcolor{red}{Delete?: However, approaches like ARIMA or RNNs suffer from the lack of model capabilities regarding non-static time series and noise~\cite{CCC}.} }

In addition to the above methods, with the proposal of the Transformer model in 2017~\cite{vaswani2017attention}, many researchers have attempted to adapt the NLP-specific Transformer architecture to the field of time series forecasting. Since the Transformer model allows modelling relationships for each point in the sequence to all previous points, it is better suited to modelling short and long term relationships than RNN-based approaches. Despite this, the canonical Transformer architecture has two weaknesses, namely its inherent locality agnostics caused by the point-wise dot product self-attention that is insensitive to local context, and its spatial complexity that grows quadratically with the length of the input sequence, thus causing a memory bottleneck in scenarios with long time series~\cite{li2019enhancing}. To address these issues, researchers have proposed many different variants of the Vanilla Transformer, where many Transformer-based solutions for time series analysis are surveyed in Wen et al.~\cite{wen2022transformers} and their effectiveness for TSF is discussed in Zeng et al.~\cite{zeng2022transformers}\todo[]{check later if both are still arXiv?}. In addition, some of the most relevant in terms of long-term time series forecasting (LTSF) and this work are presented below.

% Forecasting: 
% 1. Enhancing the Locality and Breaking the Memory Bottleneck of Transformer on Time Series Forecasting
% -> Ausführlich wie in MA
% https://proceedings.neurips.cc/paper/2019/file/6775a0635c302542da2c32aa19d86be0-Paper.pdf
In 2019, Li et al.~\cite{li2019enhancing} proposed a Transformer-based TSF architecture with the aim of adapting the long-term relationship modelling capabilities of the Transformer architecture by incorporating several changes to the vanilla Transformer. As a major modification, the authors introduced a convolutional self-attention mechanism to incorporate local context into its keys and queries. To do this, they replaced the point-wise approach of canonical self-attention with a convolutional variant, where the self-attention queries and keys are generated by a convolutional layer of kernel size $k$ based on the input. Notably, for $k=1$, this \textit{causal convolution}-based self-attention is identical to canonical self-attention and thus, represents a generalisation of it.
Aiming to tackle the quadratic space complexity, the authors also introduced \textit{sparse self-attention} as another major change to reduce the number of time points in the sequence that are considered by the attention mechanism. While Li et al. proposed different variations of sparse self-attention, the common idea behind all of them is to consider only a subset of the input sequence, selected based on some pattern. For example, the \textit{LogSparse} self-attention allows each cell to access only its predecessors with an exponential step size, while another variant puts more emphasis on the local context by allowing a cell to densely attend to its immediate predecessors while resuming LogSparse attention beyond its neighbours. In the remaining of the three variants analysed, the LogSparse approach is restarted periodically in order to cover more cells in total. 
%Regarding the remaining of the three variants analysed, Li et. al. propose to periodically restart the LogSparse approach in order to cover more cells in total. 
% Evaluating these changes
Overall, the authors reported a successful adaptation of the Transformer for TSF, reaching state-of-the-art results with the convolutional self-attention approach. 
Furthermore, the complexity could be reduced due to the sparse self-attention, while on the other hand a higher performance was obtained compared to the point-based counterpart.
% KA Robert: Furthermore, the authors reported state-of-the-art time series forecasting results with the convolutional self-attention approach and a reduction of complexity with the sparse self-attention approach with increased performance in comparison to point-wise self-attention

% 2. Informer
% -> Eher einen Überblick und darauf eingehen das hier der Transformer erstamsl für ts forecasting optimiert worder ist. Du musst aber weniger auf die spezial cases wie Probsparse eingehen. Das ist für das Paper nicht relvant
% https://ojs.aaai.org/index.php/AAAI/article/download/17325/17132
Two years later, in 2021, Zhou et al. proposed the Informer architecture, an Transformer-based model that they optimised for efficiency with respect to LTSF~\cite{zhou2021informer}. Similar to Li et al.~\cite{li2019enhancing}, they modified the vanilla Transformer architecture to improve its time complexity and memory usage, explicitly enhancing its ability to handle extremely long input sequences. The main characteristics of the adapted architecture are threefold:
First, they propose a sparse variant of self-attention, termed \textit{ProbSparse}, which aims to reduce the time complexity and memory usage of the canonical dot product-based version. 
Second, Zhou et al. established a self-attention \textit{distilling operation} to extract/privilege/favour dominating attention scores and considerably reduce the network size. 
\todo[inline]{Der naechste Satz ist sehr nah am Paper, ich habs nicht ganz durchstiegen, haette zu lange gedauert. @Robert - pls check, ggf kanns auch raus}
To improve the robustness of the distilling operation, they build replicas of the main stack with halving inputs and progressively reduce the number of self-attention distilling layers, where the concatenation of the stacks' outputs results in the final encoder representation of the input series.
Third, they introduce a decoder that operates in a generative manner, i.e., it predicts the time series sequences all at once in a single forward pass rather than in a step-wise fashion, thus resulting in an improved inference speed for long-sequence predictions.

% 3. Autoformer
% Du kannst auch eine Überleitung auf den Autoformer machen und dazu noch in zwei Sätzen schreiben was sich geändert hat. Hier kannst du einfach mal in die Seminararbeit von Michaeol schauen, der hat das hier sehr schön aufgearbeitet.
The Autoformer model was proposed by Wu et al. in the same year as the Informer, i.e., in 2021, however, despite the similarity in name, there are some substantial differences between the two architectures~\cite{wu2021autoformer}. 
~\todo[]{Der folgende Teil ist viel aus dem Paper zusammenkopiert, zwar nicht als Block aber teils sind Teilsatze fast 1:1 aus dem Paper, macht das was?}.
To begin with, although the Autoformer still follows the residual and encoder-decoder structure, it can be regarded as a deep decomposition forecasting model, since a \textit{time series decomposition} block is embedded in its architecture as a basic inner operator. This allows the Autoformer to progressively separate the long-term trend information from the predicted hidden variables, i.e. it can aggregate the long-term trend from intermediate predictions. Secondly, while Transformer-based models for LTSF, such as the Informer,  typically incorporate some form of sparse self-attention to cope with long time series, the Autoformer breaks completely with self-attention, replacing the point-wise self-attention family with an auto-correlation mechanism that focuses on series-wise connections. This mechanism finds similarities and dependencies at the sub-series level based on the periodicity of the series, and uses a so-called \textit{time delay aggregation} block to aggregate similar sub-series from underlying periods, rather than the point product-based information aggregation operation used in Transformers.
 

\subsection{Delimitation}
% Allgemein: BERT wie in der MA einfach übernehmen und etwas kürzen. Wahrscheinlich ist auch etwas Überarbeitung notwendig ;)
%  Wir machen das jetzt aber anders (cooler) und haben eine Architektur die alles auf einmal kann in dem ein TS model trainiert wird und die einzelnen Tasks weiter trainiert werden (kannst du einfach beim Approach im Motivation Part dir was klauen). Das gabs auch schon im NLP Bereich -> BERT vorstellen ähnlich wie in der MA aber deutlich gekürzt natürlich. 

In contrast to all the approaches mentioned above, which have recently been proposed for one of the three tasks of time series imputation, classification and forecasting, our architecture explicitly targets all three tasks at once, i.e. the proposed model can be used for any of the three downstream applications. To achieve this, we apply \textit{transfer learning}, a technique that refers to the process in which a model is pre-trained on a different but related task to learn contextual relationships and store knowledge that can be valuable for the subsequent downstream tasks~\cite{torrey2010transfer}. After the pre-training procedure, our generic time series model is further trained, i.e., fine-tuned, for specific tasks such as forecasting or classification without the necessity of completely retraining the model from scratch for each task.

The idea of transfer learning has already been successfully applied in the NLP domain, where it is for example used in the well-known bidirectional encoder representations from Transformers (BERT) language model by Devlin et al.~\cite{devlin2018bert}, which significantly inspired the overall concept as well as the neural network architecture of our work. Apart from the use of pre-training, the second major contribution of the BERT model was the bidirectional application of the Transformer. Using this bidirectional approach, the authors were able to show that the resulting natural language model has a deeper sense of the context of the language compared to other NLP models that rely on only one direction.
%
BERT utilizes only the encoder part of the Transformer architecture, where the same unified encoder architecture is used for both the unlabelled pre-training step for retrieving the language model and the labelled data-based fine-tuning step for learning a specific task, such as question answering. Accordingly, there are only minor differences between the pre-training and fine-tuning architectures in order to adapt the latter to the specific requirements of the downstream goal. Aiming at enabling BERT to handle a wide range of downstream tasks, a word representation layer is placed in front of the actual Transformer encoder-based BERT model to be able to model both a single sentence and a pair of sentences in one token sequence. For this purpose, the input words are pre-processed and embedded using a word embedding, where two special tokens, [CLS] and [SEP], are used to model the first word of each input sequence and to separate two sentences, respectively. To derive the final input representation that is used as input to the model, the authors introduce two further embeddings that they sum up with the  previously described embedding of each token (token embedding): A learned embedding indicating whether it belongs to the first or second sentence (segment embedding) and a third embedding representing the global position of each token in the sequence (position embedding).
%
The pre-training step of the BERT architecture learns a language model by combining two NLP-specific tasks, namely Masked Language Model (MLM) and Next Sentence Prediction (NSP), to model contextual and semantic relationships in the training corpora to build a language model. For the former, BERT learns to determine randomly masked words based on the unmasked words of the sequence, while the latter is related to a binary decision, i.e., the model is given two sentences as input and learns whether the second sentence follows the first sentence of the input sequence or not.
The language model resulting from the pre-training process can then be used in a transfer learning context for a broad range of NLP tasks by simply
adding some downstream task-specific layers to the BERT architecture, thereby significantly reducing the resource requirements for many NLP tasks, as the resource-intensive task of learning a language model only needs to be performed once. 

%Apart from borrowing the basic concept and structure from the BERT model
Apart from borrowing the main structure from the BERT model and heavily transforming it to make it suitable for time series analysis~\cite{devlin2018bert}, to the best of our knowledge, there are no approaches in the field of ANN-based time series analysis that could be described as directly related to our proposed architecture. Even though we have adopted some general ideas and individual concepts from some of the above approaches, such as the utilization of a CNN to capture local and global context for the attention layer proposed by Li et al.~\cite{li2019enhancing} or the combination of two simultaneous and interdependent tasks to enhance each other as applied in the BRITS model of Cao et el.~\cite{cao2018brits}, none of them was replicated one to one. Rather, while we have built our derived architecture on ideas from BERT, Li et al., and BRITS, we have extended them and integrated some major adaptations in order to combine them into an overall architecture with novel layers explicitly targeting the time series context.
